Development of Dual-Gain SiPM Boards for Extending the Energy Dynamic Range

Astronomical observations with gamma rays in the range of several hundred keV to hundreds of MeV currently represent the least explored energy range. To address this so-called MeV gap, we designed and built a prototype CsI:Tl calorimeter instrument using a commercial off-the-shelf (COTS) SiPMs and front-ends which may serve as a subsystem for a larger gamma-ray mission concept. During development, we observed significant non-linearity in the energy response. Additionally, using the COTS readout, the calorimeter could not cover the four orders of magnitude in energy range required for the telescope. We, therefore, developed dual-gain silicon photomultiplier (SiPM) boards that make use of two SiPM species that are read out separately to increase the dynamic energy range of the readout. In this work, we investigate the SiPM's response with regards to active area ($3\times3 \ \mathrm{mm}^2$ and $1 \times 1 \ \mathrm{mm}^2$) and various microcell sizes ($10$, $20$, and $35 \ \mu \mathrm{m}$). We read out $3\times3\times6 \ \mathrm{cm}^3$ CsI:Tl chunks using dual-gain SiPMs that utilize $35 \ \mu \mathrm{m}$ microcells for both SiPM species and demonstrate the concept when tested with high-energy gamma-ray and proton beams. We also studied the response of $17 \times 17 \times 100 \ \mathrm{mm}^3$ CsI bars to high-energy protons. With the COTS readout, we demonstrate a sensitivity to $60 \ \mathrm{MeV}$ protons with the two SiPM species overlapping at a range of around $2.5-30 \ \mathrm{MeV}$. This development aims to demonstrate the concept for future scintillator-based high-energy calorimeters with applications in gamma-ray astrophysics.

==> Hardware/dualGainSiPM.tex <==
\begin{figure}

\begin{center}



\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-0.75,xscale=0.75]
%uncomment if require: \path (0,215); %set diagram left start at 0, and has height of 215

%Image [id:dp9034282339248738] 
\draw (277.28,95.27) node [rotate=-90] {\includegraphics[width=97.68pt,height=193.85pt]{Hardware/IMG-3784.jpg}};
%Shape: Rectangle [id:dp007653626248326217] 
\draw  [color={rgb, 255:red, 251; green, 49; blue, 49 }  ,draw opacity=1 ][dash pattern={on 4.5pt off 4.5pt}] (166.81,49.19) -- (249.21,49.19) -- (249.21,137.19) -- (166.81,137.19) -- cycle ;
%Shape: Rectangle [id:dp041075359174812975] 
\draw  [color={rgb, 255:red, 133; green, 255; blue, 0 }  ,draw opacity=1 ] (192.18,75.71) -- (224.13,75.71) -- (224.13,113.88) -- (192.18,113.88) -- cycle ;
%Curve Lines [id:da39505116678740426] 
\draw [color={rgb, 255:red, 251; green, 49; blue, 49 }  ,draw opacity=1 ]   (278,190) .. controls (324.57,162.45) and (313.72,98.24) .. (254.12,68.83) ;
\draw [shift={(253.21,68.39)}, rotate = 25.8] [color={rgb, 255:red, 251; green, 49; blue, 49 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Curve Lines [id:da04317503782309151] 
\draw [color={rgb, 255:red, 133; green, 255; blue, 0 }  ,draw opacity=1 ]   (278,170) .. controls (295.51,166.82) and (299.95,92.92) .. (227.49,88.72) ;
\draw [shift={(226.39,88.67)}, rotate = 2.73] [color={rgb, 255:red, 133; green, 255; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Image [id:dp4658540932630253] 
\draw (69.83,95.04) node  {\includegraphics[width=97.75pt,height=96.94pt]{Hardware/6mmSiPM.jpg}};

% Text Node
\draw (4,16) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {{\fontfamily{pcr}\selectfont a)}};
% Text Node
\draw (144,16) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {{\fontfamily{pcr}\selectfont b)}};
% Text Node
\draw (141,179) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\fontfamily{cmr}\selectfont high gain (9 mm}$\displaystyle ^{2}${\fontfamily{cmr}\selectfont )}};
% Text Node
\draw (141,160) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{82.02pt}\setlength\topsep{0pt}
\begin{flushright}
{\fontfamily{cmr}\selectfont low gain (1 mm}$\displaystyle ^{2}${\fontfamily{cmr}\selectfont )}
\end{flushright}

\end{minipage}};


\end{tikzpicture}




\end{center}


  \caption{(a) SensL/onsemi Quad-SiPM design utilized in the ComPair CsI calorimeter prototype. (b) The NRL custom design dual-gain SiPM with the low-gain group outlined in the solid green while the high-gain group is outlined in the dashed red.}
  \label{fig:dualGainSiPM}
\end{figure}

